The chiral transition and U(1)_A symmetry restoration from lattice QCD using Domain Wall Fermions

We present results on both the restoration of the spontaneously broken chiral symmetry and the effective restoration of the anomalously broken U(1)_A symmetry in finite temperature QCD at zero chemical potential using lattice QCD. We employ domain wall fermions on lattices with fixed temporal extent N_\tau = 8 and spatial extent N_\sigma = 16 in a temperature range of T = 139 - 195 MeV, corresponding to lattice spacings of a \approx 0.12 - 0.18 fm. In these calculations, we include two degenerate light quarks and a strange quark at fixed pion mass m_\pi = 200 MeV. The strange quark mass is set near its physical value. We also present results from a second set of finite temperature gauge configurations at the same volume and temporal extent with slightly heavier pion mass. To study chiral symmetry restoration, we calculate the chiral condensate, the disconnected chiral susceptibility, and susceptibilities in several meson channels of different quantum numbers. To study U(1)_A restoration, we calculate spatial correlators in the scalar and pseudo-scalar channels, as well as the corresponding susceptibilities. Furthermore, we also show results for the eigenvalue spectrum of the Dirac operator as a function of temperature, which can be connected to both U(1)_A and chiral symmetry restoration via Banks-Casher relations.

==> normalization.tex <==
\subsection{Normalization conventions}

By using the methods described above, we can easily adopt a 
common normalization convention for the quark mass, chiral
condensate and Dirac spectrum.  This allows a meaningful comparison 
between features of the Dirac spectrum and the corresponding 
value of the quark mass which may be the origin of those 
features.  Given the central role which is played by both the 
quark mass and the Dirac eigenvalue spectrum in the physics of 
finite temperature QCD, it seems sensible to adopt a normalization 
scheme that is the current standard used in continuum physics and 
one in which the physical quark masses are often presented, 
the $\overline{\rm MS}$ scheme, normalized at a scale $\mu=2$ GeV.  
Quantities which we present in this scheme can be easily converted 
to other popular normalization schemes such as $\overline{\rm MS}$ 
for a larger value of $\mu$, the non-perturbative RI scheme or the 
RGI scheme by the application of standard perturbation theory 
formulae.  Quark masses given in this scheme can also be directly
compared with other finite temperature studies performed with 
different fermion actions, provided those results are also cast
into this conventional scheme.

We will use the DWF results for the continuum, $\mu=2$ GeV, 
$\overline{\rm MS}$ quark masses determined in 
Ref.~\cite{Aoki:2010dy}, 
$m^{\overline{\rm MS}}_s(2\;{\rm GeV}) = (96.2 \pm 2.7)$MeV and 
$m^{\overline{\rm MS}}_{ud}(2\;{\rm GeV}) = (3.59\pm0.21)$MeV and
the accurate linear dependence of $m_\pi^2$ and $m_K^2$ on the quark 
masses in the region studied to convert a lattice light quark mass, 
$\widetilde{m}_l=m_f+m_{\rm res}$ corresponding to a pion mass 
$m_\pi(\widetilde{m}_l)$ into this same $\overline{\rm MS}$
scheme using the relation:
\begin{equation}
m^{\overline{\rm MS}}_l(2{\rm GeV}) 
                 = (3.59 + 96.2) \mbox{MeV} 
               \frac{\Bigl(m_\pi(\widetilde{m}_l)\Bigr)^2}{2(495 MeV)^2}.
\end{equation}
Making the assumption that our choice of quark mass at each
value of $\beta$ lies on a line of constant physics with
$m_\pi = 200$ MeV, we can compute the needed renormalization
factor:
\begin{equation}
Z_{m_f \to \overline{\rm MS}} = \frac{99.79 MeV}{2\widetilde{m}} 
                             \left(\frac{200}{495}\right)^2
\label{eq:Z_mf_MSbar}
\end{equation}
for each of our ensembles.  Note the lattice quark mass, $\widetilde{m}$,
substituted in Eq.~\ref{eq:Z_mf_MSbar} must be expressed in units of MeV to 
define a conventional, dimensionless value for $Z_{m_f \to \overline{\rm MS}}$. 
The resulting $Z_{m_f \to \overline{\rm MS}}$ factors for our seven ensembles 
are given in Tab.~\ref{tab:Z_MS_bar}.  By assumption, all of the light quark 
masses in our simulation have the common, $\mu=2$ GeV, $\overline{\rm MS}$ 
value of 16.3 MeV.  

\begin{table}[H]
\begin{center}
\begin{tabular}{lc}
\hline
$T$ (MeV)   & $Z_{m_f \to \overline{\rm MS}}(2 \mbox{MeV})$ \\ 
\hline
140  &  2.83 \\
150  &  2.91 \\
160  &  2.79 \\
170  &  3.03 \\
180  &  3.10 \\
190  &  3.14 \\
200  &  3.20 \\
\hline
\end{tabular}
\end{center}
\caption{Results for the factors $Z_{m_f \to \overline{\rm MS}}(2 \mbox{GeV})$ 
which convert a lattice quark mass, $\widetilde{m}$ into a mass normalized in 
the $\overline{\rm MS}$ conventions at $\mu=2$ GeV.}
\label{tab:Z_MS_bar}
\end{table}

The factors given in Tab.~\ref{tab:Z_MS_bar} will also be used to convert 
values of the chiral condensate $\overline{q}q$ (when constructed the usual 
4-D surface, lattice operators) and Dirac spectrum (when normalized with the 
same conventions as $\overline{q}q$) into $\mu =2$ GeV, $\overline{\rm MS}$ 
values according to the relations:
\begin{eqnarray}
(\overline{q}q)^{\overline{\rm MS}}
             &=& \frac{(\overline{q}q)^{\rm lat}}{Z_{m_f \to \overline{\rm MS}}} \\
\rho(\lambda)^{\overline{\rm MS}}
             &=& \frac{\rho^{\rm lat}(\lambda/Z_{m_f \to \overline{\rm MS}})}
                 {Z_{m_f \to \overline{\rm MS}}}.
\end{eqnarray}
Note in these equations we are converting dimensionfull quantities from
one normalization scheme to another.  Each carries the appropriate physical
dimension whose units need not be specified here.  The quantities 
$(\overline{q}q)^x$ and $\rho(\lambda)^x$, have units of (energy$)^3$ while 
$\lambda$ carries units of energy.  These may be expressed in lattice units 
or in GeV as appropriate.

We could compute more accurate values for the factors given 
Tab.~\ref{tab:Z_MS_bar} by performing a zero temperature calculation
at each of our seven $\beta$ values and determining the lattice scale 
and the pion mass for the quark masses that are used.  However, for
the purposes of the present paper, we believe the conversion factors
in Tab.~\ref{tab:Z_MS_bar} have sufficient accuracy.


==> renorm.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,660){\makebox(0,0)[r]{\strut{} 1}}%
      \put(-132,1404){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(-132,2148){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(-132,2891){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(-132,3635){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(-132,4379){\makebox(0,0)[r]{\strut{} 2}}%
      \put(0,440){\makebox(0,0){\strut{} 0}}%
      \put(756,440){\makebox(0,0){\strut{} 1}}%
      \put(1511,440){\makebox(0,0){\strut{} 2}}%
      \put(-902,2519){\rotatebox{-270}{\makebox(0,0){\strut{}$ Z_{\mathrm{tw}\to m_f}$}}}%
      \put(1133,110){\makebox(0,0){\strut{}$ (ap)^2$}}%
      \put(756,4007){\makebox(0,0)[l]{\strut{}$ \beta =1.70$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1280,1548){\makebox(0,0)[r]{\strut{}$ \mathcal{R}^\mathrm{non-ex}_\mathrm{MOM}$}}%
      \csname LTb\endcsname%
      \put(1280,1218){\makebox(0,0)[r]{\strut{}$ \mathcal{R}^\mathrm{ex}_\mathrm{MOM}$}}%
      \csname LTb\endcsname%
      \put(1280,888){\makebox(0,0)[r]{\strut{}$ \mathcal{R}_{\pi}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2268,660){\makebox(0,0)[r]{\strut{}}}%
      \put(2268,1404){\makebox(0,0)[r]{\strut{}}}%
      \put(2268,2148){\makebox(0,0)[r]{\strut{}}}%
      \put(2268,2891){\makebox(0,0)[r]{\strut{}}}%
      \put(2268,3635){\makebox(0,0)[r]{\strut{}}}%
      \put(2268,4379){\makebox(0,0)[r]{\strut{}}}%
      \put(2400,440){\makebox(0,0){\strut{} 0}}%
      \put(3156,440){\makebox(0,0){\strut{} 1}}%
      \put(3911,440){\makebox(0,0){\strut{} 2}}%
      \put(3533,110){\makebox(0,0){\strut{}$ (ap)^2$}}%
      \put(3156,4007){\makebox(0,0)[l]{\strut{}$ \beta =1.75$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4668,660){\makebox(0,0)[r]{\strut{}}}%
      \put(4668,1404){\makebox(0,0)[r]{\strut{}}}%
      \put(4668,2148){\makebox(0,0)[r]{\strut{}}}%
      \put(4668,2891){\makebox(0,0)[r]{\strut{}}}%
      \put(4668,3635){\makebox(0,0)[r]{\strut{}}}%
      \put(4668,4379){\makebox(0,0)[r]{\strut{}}}%
      \put(4800,440){\makebox(0,0){\strut{} 0}}%
      \put(5556,440){\makebox(0,0){\strut{} 1}}%
      \put(6311,440){\makebox(0,0){\strut{} 2}}%
      \put(5933,110){\makebox(0,0){\strut{}$ (ap)^2$}}%
      \put(5556,4007){\makebox(0,0)[l]{\strut{}$ \beta =1.82$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./figs/renorm}}%
    \gplfronttext
  \end{picture}%
\endgroup

